Multi-view Local Co-occurrence and Global Consistency Learning Improve Mammogram Classification Generalisation

When analysing screening mammograms, radiologists can naturally process information across two ipsilateral views of each breast, namely the cranio-caudal (CC) and mediolateral-oblique (MLO) views. These multiple related images provide complementary diagnostic information and can improve the radiologist's classification accuracy. Unfortunately, most existing deep learning systems, trained with globally-labelled images, lack the ability to jointly analyse and integrate global and local information from these multiple views. By ignoring the potentially valuable information present in multiple images of a screening episode, one limits the potential accuracy of these systems. Here, we propose a new multi-view global-local analysis method that mimics the radiologist's reading procedure, based on a global consistency learning and local co-occurrence learning of ipsilateral views in mammograms. Extensive experiments show that our model outperforms competing methods, in terms of classification accuracy and generalisation, on a large-scale private dataset and two publicly available datasets, where models are exclusively trained and tested with global labels.

==> backup_table.tex <==
\begin{table}
    % \parbox{.45\linewidth}{
    \begin{minipage}[t]{.5\linewidth}
        \centering
        % \caption{Foo}
        \begin{tabular}{c|c|c}
        \toprule
            Methods	    &	ADMANI1	&	ADMANI2 \\ \midrule\midrule
            Baseline	&	88.61	&	87.51   \\
            GMIC~\cite{shen2021interpretable}	    &	88.89	&	N/A     \\
            DMV-CNN~\cite{shen2019deep}	    &	N/A	    &	N/A     \\
            MVCCL	    &	94.78	&	92.52   \\ \hline\bottomrule
        \end{tabular}
        \caption{sssssss}
    % }
    \end{minipage}%
    % \quad
    \begin{minipage}[t]{.5\linewidth}
    % \parbox{.45\linewidth}{
        \centering
        \begin{tabular}{cccc|c}
        \toprule%\hline
            Fusion 	    & SA               &	LCL	         	&	GCL	            &	Testing AUC \\\midrule\midrule%\hline \hline
            % \checkmark	&		           &	                &	                &	88.61	\\
            \checkmark	&		           &	                &	                &	90.88   \\
            \checkmark	&	\checkmark     &			        &		            &	92.53	\\
            \checkmark	&	               &	\checkmark	    &		            &	93.68	\\
            \checkmark	&	               &		            &	\checkmark	    &	92.41	\\
            \checkmark	&	\checkmark     &		            &	\checkmark	    &	93.53	\\
            \checkmark	&   \checkmark     &	\checkmark	    &	\checkmark	    &	\red{\textbf{94.78}}	\\ \hline\bottomrule
        \end{tabular}%
        \caption{\textbf{Baseline}: EfficientNet-b0. \textbf{Fusion}: concatenate the output feature vector of two views. \textbf{Data Augmentation}: perform random affine transformation to the input image}
    % }
    \end{minipage}%

    \end{table}
    
    
    
    
    
    \begin{table}
    % \parbox{.45\linewidth}{
    \begin{minipage}[t]{.5\linewidth}
        \centering
        % \caption{Foo}
        \begin{tabular}{c|c|c}
        \toprule
            Methods	    &	ADMANI1	&	ADMANI2 \\ \midrule\midrule
            Baseline	&	88.61	&	87.51   \\
            GMIC~\cite{shen2021interpretable}	    &	88.89	&	N/A     \\
            DMV-CNN~\cite{shen2019deep}	    &	N/A	    &	N/A     \\
            MVCCL	    &	94.78	&	92.52   \\ \hline\bottomrule
        \end{tabular}
        \caption{sssssss}
    % }
    \end{minipage}%
    % \quad
    \begin{minipage}[t]{.5\linewidth}
    % \parbox{.45\linewidth}{
        \centering
        \begin{tabular}{cccc|c}
        \toprule%\hline
            Fusion 	    & SA               &	LCL	         	&	GCL	            &	Testing AUC \\\midrule\midrule%\hline \hline
            % \checkmark	&		           &	                &	                &	88.61	\\
            \checkmark	&		           &	                &	                &	90.88   \\
            \checkmark	&	\checkmark     &			        &		            &	91.83	\\
            \checkmark	&	               &	\checkmark	    &		            &	93.68	\\
            \checkmark	&	               &		            &	\checkmark	    &	92.41	\\
            \checkmark	&	\checkmark     &		            &	\checkmark	    &	93.53	\\
            \checkmark	&   \checkmark     &	\checkmark	    &	\checkmark	    &	\red{\textbf{94.78}}	\\ \hline\bottomrule
        \end{tabular}%
        \caption{\textbf{Baseline}: EfficientNet-b0. \textbf{Fusion}: concatenate the output feature vector of two views. \textbf{Data Augmentation}: perform random affine transformation to the input image}
    % }
    \end{minipage}%

    \end{table}

==> minpage_table.tex <==
% \begin{table}[t]
% \centering
% \vspace{-20pt}
% % \caption{}
% \captionsetup{width=.8\textwidth}
% \resizebox{.85\textwidth}{!}{
% \begin{subtable}[t]{0.5\textwidth}
% \centering
% \vspace{-5pt}

% \caption{Image-level mean and 95\% CI AUC-ROC results for ANON datasets.}\vspace{-1pt}
% \label{tab:ablation}
% \resizebox{\textwidth}{!}{\begin{tabular}{!{\vrule width 1pt}c|cc}
% \specialrule{1pt}{0pt}{0pt}
% % \toprule
% Methods	                                    &	ANON-1 (test set)	                &	ANON-2 (whole set)                \\ \midrule\midrule
% EfficientNet-b0~\cite{tan2019efficientnet}	&	\makecell{88.61\\(87.30-89.00)} 	&	\makecell{83.77\\(82.80-84.70)}   \\ \hline
% DMV-CNN~\cite{shen2019deep}	                &	\makecell{80.23\\(76.20-85.31)}	    &	\makecell{n/a\\(-)}     \\ \hline
% GMIC~\cite{shen2021interpretable}	        &	\makecell{88.89\\(-)}	&	\makecell{\\(-)}     \\ \hline
% MVCCL	                                    &	\makecell{94.78\\(93.66-95.27)}   &	\makecell{92.60\\(92.17-92.99)}   \\ \hline\bottomrule
% \specialrule{1pt}{0pt}{0pt}
% \end{tabular}}
% \end{subtable} \hfill
% \begin{subtable}[t]{0.5\textwidth}
% \vspace{-5pt}
% \centering
% \caption{Ablation study of key components of our MVCCL model.} \vspace{-2pt}
% \label{tab:loss_ablation}
% \resizebox{\textwidth}{!}
% {\begin{tabular}{c|c|c|c|c} 
% \specialrule{1pt}{0pt}{0pt}
% % \toprule%\hlines
% Fusion 	    & SA               &	LCM	         	&	GCM	            &	Testing AUC \\\midrule\midrule%\hline \hline
% % \checkmark	&		           &	                &	                &	88.61	\\
% \checkmark	&		           &	                &	                &	90.88   \\
% \checkmark	&	\checkmark     &			        &		            &	91.83	\\
% \checkmark	&	               &	\checkmark	    &		            &	93.68	\\
% \checkmark	&	               &		            &	\checkmark	    &	92.41	\\
% \checkmark	&	\checkmark     &		            &	\checkmark	    &	93.53	\\
% \checkmark	&                  &	\checkmark	    &	\checkmark	    &	\textbf{94.78}	\\
% % \hline\bottomrule
% \specialrule{1pt}{0pt}{0pt}
% \end{tabular}}
% \end{subtable}
% }
% \end{table}



% \begin{table}[t]
% % \parbox{.45\linewidth}{
% \centering
% \caption{Image-level mean and 95\% CI AUC-ROC results for ANON datasets.}
% \begin{tabular}{P{3cm}|P{2cm}P{2cm}}
% \toprule
%     Methods	                                    &	ANON-1 (test set)	                &	ANON-2 (whole set)                \\ \midrule\midrule
%     EfficientNet-b0~\cite{tan2019efficientnet}	&	\makecell{88.61\\(87.30-89.00)} 	&	\makecell{83.77\\(82.80-84.70)}   \\ \hline
%     DMV-CNN~\cite{shen2019deep}	                &	\makecell{80.23\\(76.20-85.31)}	    &	\makecell{n/a\\(-)}     \\ \hline
%     GMIC~\cite{shen2021interpretable}	        &	\makecell{88.89\\(-)}	&	\makecell{\\(-)}     \\ \hline
%     MVCCL	                                    &	\makecell{94.78\\(93.66-95.27)}   &	\makecell{92.60\\(92.17-92.99)}   \\ \hline\bottomrule
% \end{tabular}
% \label{tab:admani}
% \end{table}



% \begin{table}[t]
%     \centering
%     \caption{Ablation study of key components of our MVCCL model.}
%     % \scalebox{0.9}{
%     % \resizebox{\linewidth}{!}{%
%     \begin{tabular}{ c c c c | c}
%     \toprule%\hlines
%         Fusion 	    & SA               &	LCM	         	&	GCM	            &	Testing AUC \\\midrule\midrule%\hline \hline
%         % \checkmark	&		           &	                &	                &	88.61	\\
%         \checkmark	&		           &	                &	                &	90.88   \\
%         \checkmark	&	\checkmark     &			        &		            &	91.83	\\
%         \checkmark	&	               &	\checkmark	    &		            &	93.68	\\
%         \checkmark	&	               &		            &	\checkmark	    &	92.41	\\
%         \checkmark	&	\checkmark     &		            &	\checkmark	    &	93.53	\\
%         \checkmark	&                  &	\checkmark	    &	\checkmark	    &	\textbf{94.78}	\\ \hline\bottomrule
%     \end{tabular}%
%     \label{tab:ablation}
%     % \caption{\textbf{Baseline}: EfficientNet-b0. \textbf{Fusion}: concatenate the output feature vector of two views. \textbf{Data Augmentation}: perform random affine transformation to the input image}
%     % }
% \end{table}


\begin{table}[t]
\begin{minipage}[t]{0.48\linewidth}\centering
    \resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{c|cc}
    \toprule
        Methods	                                    &	\makecell{ANON-1\\(test set)}	                &	\makecell{ANON-2\\(whole set)}                \\ \midrule\midrule
        EfficientNet-b0~\cite{tan2019efficientnet}	&	\makecell{88.61\\(87.30-89.00)} 	&	\makecell{83.77\\(82.80-84.70)}   \\ \hline
        DMV-CNN~\cite{shen2019deep}	                &	\makecell{80.23\\(76.20-85.31)}	    &	\makecell{n/a\\(-)}     \\ \hline
        GMIC~\cite{shen2021interpretable}	        &	\makecell{88.89\\(-)}	&	\makecell{\\(-)}     \\ \hline
        MVCCL	                                    &	\makecell{94.78\\(93.66-95.27)}   &	\makecell{92.60\\(92.17-92.99)}   \\ \hline\bottomrule
    \end{tabular}
    }
\caption{Image-level mean and 95\% CI AUC-ROC results for ANON datasets.}
\label{tab:admani}
\end{minipage}
\hspace{0.04cm}
\begin{minipage}[t]{0.48\linewidth}
    \centering
    % \resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{ c|c|c|c|c}
    \toprule%\hlines
        Fusion 	    & SA               &	LCM	         	&	GCM	            &	Testing AUC \\\midrule\midrule%\hline \hline
        % \checkmark	&		           &	                &	                &	88.61	\\
        \checkmark	&		           &	                &	                &	90.88   \\
        \checkmark	&	\checkmark     &			        &		            &	91.83	\\
        \checkmark	&	               &	\checkmark	    &		            &	93.68	\\
        \checkmark	&	               &		            &	\checkmark	    &	92.41	\\
        \checkmark	&	\checkmark     &		            &	\checkmark	    &	93.53	\\
        \checkmark	&                  &	\checkmark	    &	\checkmark	    &	\textbf{94.78}	\\ \hline\bottomrule
    \end{tabular}%
\caption{Ablation study of key components of our MVCCL model.}
\label{tab:ablation}
    % }
\end{minipage}
\end{table}




==> package.tex <==
% \usepackage[utf8]{inputenc}
\usepackage{geometry}
% \geometry{left=1in,top=2.25in}
% \setlength{\parindent}{0em}
% \setlength{\parskip}{1em}
\usepackage{graphicx}


\usepackage{epsfig}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}
\usepackage{ dsfont }
\usepackage{ cite }
\usepackage{float}
\usepackage{color}
\usepackage{xcolor}
\usepackage{soul}
\usepackage{float}
\usepackage{url}
% \usepackage{caption}
% \usepackage{subcaption}
\usepackage{rotate}
\usepackage{tikz}
\usepackage[colorlinks=true, citecolor=blue]{hyperref}%


\newcommand{\yuanhong}[1]{\textcolor{orange}{Yuanhong: #1}}
\newcommand{\gustavo}[1]{\textcolor{red}{Gustavo: #1}}


\newcommand{\red}[1]{\textcolor{red}{#1}}
